Position-dependence of valley polarization and valley coherence of WS2 monolayer flakes

Chiral interaction between light and two-dimensional transition metal dichalcogenides (2D-TMDs) has recently drawn enormous scientific attention. The optical selection rules of these atomically thin semiconductors allow the attribution of a pseudospin to the TMDs' valleys, which can be coherently manipulated for information processing using polarized light. The interaction of TMDs with circularly and linearly polarized light creates the valley polarization and coherence, respectively. With a full Stokes polarization analysis of light emitted from WS2 monolayer flakes, we conclusively confirm the existence of coherence between its valleys. We observe spatial heterogeneity in photoluminescence intensity, valley polarization and valley coherence. The discovery of an inverse proportional relationship between photoluminescence intensity and both valley polarization and coherence, reveals a correlation between the (non-)radiative decay rate and the valley hopping. The temperature dependence confirms the phononic nature of valley depolarization and decoherence, that may be caused by strain and the presence of defects.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
